High Performance W-stacking for Imaging Radio Astronomy Data: a Parallel and Accelerated Solution

Current and upcoming radio-interferometers are expected to produce volumes of data of increasing size that need to be processed in order to generate the corresponding sky brightness distributions through imaging. This represents an outstanding computational challenge, especially when large fields of view and/or high resolution observations are processed. We have investigated the adoption of modern High Performance Computing systems specifically addressing the gridding, FFT-transform and w-correction of imaging, combining parallel and accelerated solutions. We have demonstrated that the code we have developed can support dataset and images of any size compatible with the available hardware, efficiently scaling up to thousands of cores or hundreds of GPUs, keeping the time to solution below one hour even when images of the size of the order of billion or tens of billion of pixels are generated. In addition, portability has been targeted as a primary objective, both in terms of usability on different computing platforms and in terms of performance. The presented results have been obtained on two different state-of-the-art High Performance Computing architectures.

==> referee_replies.tex <==
The authors want to thank the reviewer for the useful comments and suggestions that have strongly helped in improving the manuscript in terms of clarity and completeness. The main changes to the original text have been highlighted in the new version in bold. Answers to the specific requests by the reviewer follow.

Q: 1- The correlation the authors compute appears to be 2D (from Eq.(6)), which matches some of the datasets used, although not others. In particular, galaxy surveys and HI maps will be tomographic, so why isn't the 3D correlation also computed?
A: In the paper, our target is to analyse the cross-correlation between different quantities, giving guidelines to potential observational campaigns. In particular, we aim at creating realistic mock observations, reproducing what can be measured with different instruments. Therefore it is natural to limit to 2D imaging, which is expected to be available in all the different cases, with final data products (the images) that can be directly compared and cross-correlated.
Including in the analysis 3D data is potentially of great interest, but it implies extending substantially the implemented methodology. In particular, HI data cube axes are not homogeneous, the "third" dimension not being spatial. This requires an additional step of reworking the simulated data in order to mimic observations with the necessary degree of "realism". This is a particularly delicate task, that we consider to go beyond the objectives of the current paper.
However, we have calculated the cross-correlation between the 3D DM and HI distributions for the CSFBH2 model (the only model with self-consistent description of HI). The correlation is computed for sub-boxes of size 200^3 cells, in order to have sufficient statistics and to keep the computational requirements reasonable (larger boxes needs big CPU resources). The results (Figure Rev1, attached to this reply) show that the 3D correlation (solid green line, compared to the corresponding null model, dashed line) is substantially the same as in 2D (shown in Figure 11 in the paper).

Q: 2- The authors correlate every observable with the DM distribution, but that is not the most readily observable field. Surveys will map galaxies, so why not cross correlate with those?
A: As pointed out in the paper, our simulations are not suitable to treat galaxy formation, hence we preferred to avoid any direct reference to galaxies, considering only Dark Matter and halos, the latter considered representative of galaxies. 
Figure 10 shows the correlation between the Dark Matter distribution and its highest peaks where halos are expected to form. Additionally, we provide in Figure Rev2 (attached to this reply) the cross-correlation of the DM with the halo catalogues calculated in Gheller C., Vazza F., Brueggen M., Alpaslan M., Holwerda B. W.,Hopkins A. M., Liske J., 2016, MNRAS, 462, 448, that are limited to the halo population in filaments. 
Both figures show a good degree of correlation between the DM and the halo distribution. That is why we decided to adopt directly the DM as a reliable tracer of the halo distribution in the calculation of the cross-correlation with other quantities.


I also have some minor comments:

Q: -The authors should cite:
https://arxiv.org/abs/1709.10378
as well as
https://arxiv.org/abs/1709.05024
where cross correlation of SZ maps with galaxy surveys detected the WHIM for the first time.
A: Done (in the introduction). 

Q: -the SZ "decrement" is not always a decrement, it depends on the observable frequency. Likewise for the 21-cm signal (as at low-z it's emission, not absorption). I'd change it to SZ/21-cm signal. 
A: Good point, we changed our text accordingly. 


Q:-The abstract talks about "radio observables", please expand. 
A: done

Q:-I enjoyed the introduction, just FYI.
A: Thanks.

Q: -Please define all symbols as soon as they appear in eqs. especially in Eq. (2).
A: Done.

Q:-In page 5, line 14, explain why a 10^(-6) fraction is used.
A: Done in the text.

Q:-Page 5, line 41, why is a spherical model used? Why not track the actual halo profile with the simulation?
A: It is indeed what we did, this is better explained now in the text. 

Q:-What is being correlated in Fig. 7?
A:  Figure 7 shows the two point correlation function of the halos extracted in the different runs from the filaments. The procedure is explained in details in Gheller C., Vazza F., Brueggen M., Alpaslan M., Holwerda B. W.,Hopkins A. M., Liske J., 2016, MNRAS, 462, 448. The goal was to show that the statistical properties of our halos are compatible with those in the literature (as done in section 2 for the other quantities presented in the paper).

Q:-In page 7, line 43 left, please elaborate on what we are supposed to learn from Fig. 8.
A: Done in the text.

Q: -Figure 8, and the rest of C_r plots. I'd change the axes to logplot, as in Fig. 7, which more clearly shows the range and difference between curves (with abs() when necessary). 
A: We tried to use log scales on both axis. We found that the log scale on the y axis tends to highlight the part of the correlation curve at large displacements, emphasising random differences while damping the relevant ones toward 0. The log scale on the x-axis tends to give to much emphasis to the very first bins, close to 0, while we are focusing on displacements around 1 Mpc. Two examples are provided in attachment (figures Rev3 and Rev4). For these reasons, we prefer to keep the image in linear scale. 

Q:-Also, if the three sims have the same I.C.s it might be useful to show the correlation between them.
A: The authors are not sure of the meaning of the request. Is the reviewer asking to cross-correlate the same quantity among different simulations (e.g. DM distribution from the three models) to estimate the impact of the different physical models starting from the same initial conditions (which in fact are exactly the same)? This is for sure an interesting question but we think that it is outside the scope of the paper, which intends to give guidelines to potential observations.  

Q: -Fig. 9, why are the last two rows so different between the simulations? Explain in caption or text. (also, isn't it CSFBH2? why is it labeled as 5 in the figure?)
A: It was a typo, we corrected it in the new version (and also updated the color palette of all panels in the figure)

Q: -In FIg. 10 and subsequent I'd move the \Delta \theta from the bottom of the plot to the top, where it belongs.
A: Done

Q: -In Fig. 15, rescaled 100 times... lower or higher? clarify
A: Lower; clarified in the revised text. 

==> todo.tex <==
- risolvere masking strutture non mascherate
- masking con tagli di massa (galssie vs no galassie)
- dividere sky models in quadrati di 4 x 4 tiles 
- 
